DeepShapeMatchingKit: Accelerated Functional Map Solver and Shape Matching Pipelines Revisited

Deep functional maps, leveraging learned feature extractors and spectral correspondence solvers, are fundamental to non-rigid 3D shape matching. Based on an analysis of open-source implementations, we find that standard functional map implementations solve k independent linear systems serially, which is a computational bottleneck at higher spectral resolution. We thus propose a vectorized reformulation that solves all systems in a single kernel call, achieving up to a 33x speedup while preserving the exact solution. Furthermore, we identify and document a previously unnoticed implementation divergence in the spatial gradient features of the mainstay DiffusionNet: two variants that parameterize distinct families of tangent-plane transformations, and present experiments analyzing their respective behaviors across diverse benchmarks. We additionally revisit overlap prediction evaluation for partial-to-partial matching and show that balanced accuracy provides a useful complementary metric under varying overlap ratios. To share these advancements with the wider community, we present an open-source codebase, DeepShapeMatchingKit, that incorporates these improvements and standardizes training, evaluation, and data pipelines for common deep shape matching methods. The codebase is available at: https://github.com/xieyizheng/DeepShapeMatchingKit

==> 06_instructions.tex <==
\section{Instructions}


==> figs/pck_tikz/geo_errors_plain_becos.tex <==
\addlegendentry{\textcolor{black}{DPFM \textbf{62.35} / 48.18 }}
\addlegendentry{\textcolor{black}{EchoMatch 60.13 / \textbf{52.40} }}
\addplot [color=cPLOT_dpfm, solid, smooth, line width=\pckLineWidth]
table[row sep=crcr]{%
0.0  0.7772352398249323\\
0.01  1.5575966891952242\\
0.02  4.35406556108018\\
0.03  7.908714681275493\\
0.04  11.883466817518682\\
0.05  15.864322505731385\\
0.06  19.74662815970465\\
0.07  23.33075296989907\\
0.08  26.511150147378448\\
0.09  29.302855271384765\\
0.1  31.691874832524487\\
0.11  33.64307619019263\\
0.12  35.236549855598895\\
0.13  36.59659987495162\\
0.14  37.70982820734213\\
0.15  38.62372346443564\\
0.16  39.41599428350255\\
0.17  40.09944323696668\\
0.18  40.68597969452467\\
0.19  41.222347932235685\\
0.2  41.69053502843362\\
0.21  42.084437431148956\\
0.22  42.45764730401643\\
0.23  42.78962098430941\\
0.24  43.104474945663505\\
0.25  43.39506356626075\\
0.26  43.63786584095037\\
0.27  43.86473933367077\\
0.28  44.047101557150086\\
0.29  44.24479709411379\\
0.3  44.42745705183553\\
0.31  44.57811057849763\\
0.32  44.73055051061422\\
0.33  44.854705689701376\\
0.34  44.99940453151517\\
0.35  45.12430404620835\\
0.36  45.240718134992704\\
0.37  45.35683448953464\\
0.38  45.47280197695537\\
0.39  45.57849763301277\\
0.4  45.67079524816149\\
0.41  45.75862684967398\\
0.42  45.84362997588352\\
0.43  45.93041950754756\\
0.44  46.01765564057522\\
0.45  46.09789501890613\\
0.46  46.1776877958734\\
0.47  46.251972489356\\
0.48  46.32953225950517\\
0.49  46.40485902283621\\
0.5  46.4769107095007\\
0.51  46.55342840980141\\
0.52  46.63083931282937\\
0.53  46.70318873373627\\
0.54  46.76869026706761\\
0.55  46.82287789918719\\
0.56  46.87632119570072\\
0.57  46.92812695388097\\
0.58  46.97933724357639\\
0.59  47.0286122606961\\
0.6  47.0755054038765\\
0.61  47.12820436478399\\
0.62  47.175097507964395\\
0.63  47.21975764432668\\
0.64  47.262780242355674\\
0.65  47.303123232202935\\
0.66  47.34703903295918\\
0.67  47.38559561735195\\
0.68  47.43248876053235\\
0.69  47.472534016137196\\
0.7  47.50707118825736\\
0.71  47.54622324113496\\
0.72  47.591032244618454\\
0.73  47.6407538631018\\
0.74  47.6779706434037\\
0.75  47.71101914431179\\
0.76  47.737219757644326\\
0.77  47.762824902492035\\
0.78  47.790514187036656\\
0.79  47.808824842945185\\
0.8  47.82728436597493\\
0.81  47.848125762943994\\
0.82  47.86718075445857\\
0.83  47.88489594188228\\
0.84  47.906183940214966\\
0.85  47.92896060975973\\
0.86  47.94771786703188\\
0.87  47.967814928394915\\
0.88  47.98925179384881\\
0.89  48.01173072915116\\
0.9  48.03867567808974\\
0.91  48.06591836127073\\
0.92  48.09226784172448\\
0.93  48.11608658111769\\
0.94  48.136183642480724\\
0.95  48.164170661267754\\
0.96  48.18396998838836\\
0.97  48.20510911959984\\
0.98  48.218804894750946\\
0.99  48.23458480959895\\
1.0  48.248131717628844\\
1.01  48.262869562628396\\
1.02  48.27537440080984\\
1.03  48.285646232173164\\
1.04  48.29919314020306\\
1.05  48.31497305505106\\
1.06  48.326286956262834\\
1.07  48.3373031232322\\
1.08  48.3469794861107\\
1.09  48.36097299550421\\
1.1  48.370500491261495\\
1.11  48.38255872807932\\
1.12  48.393426027927475\\
1.13  48.39938071277577\\
1.14  48.405633131866495\\
1.15  48.41203441807843\\
1.16  48.415756096108616\\
1.17  48.420966445350885\\
1.18  48.42677226307798\\
1.19  48.432280346562656\\
1.2  48.43763956292613\\
1.21  48.44329651353202\\
1.22  48.4467204573198\\
1.23  48.45237740792568\\
1.24  48.45565248459226\\
1.25  48.45833209277399\\
1.26  48.46800845565248\\
1.27  48.4742608747432\\
1.28  48.480215559591514\\
1.29  48.48617024443981\\
1.3  48.491231726560876\\
1.31  48.49882394974246\\
1.32  48.501503557924195\\
1.33  48.5074582427725\\
1.34  48.51162652216631\\
1.35  48.512817459135974\\
1.36  48.51594366868133\\
1.37  48.51817667549945\\
1.38  48.520856283681184\\
1.39  48.524280227468964\\
1.4  48.52681096852949\\
1.41  48.528597373983985\\
1.42  48.529490576711225\\
1.43  48.53023491231727\\
1.44  48.531276982165714\\
1.45  48.53157471640813\\
1.46  48.53202131777176\\
1.47  48.53261678625659\\
1.48  48.53306338762021\\
1.49  48.53350998898383\\
    };
\addplot [color=cPLOT_ours, solid, smooth, line width=\pckLineWidth]
table[row sep=crcr]{%
0.0  0.393455668609852\\
0.01  1.3276445187431747\\
0.02  3.7022618333688766\\
0.03  6.624768671253404\\
0.04  9.800896260238936\\
0.05  13.024685085181936\\
0.06  16.188646893217363\\
0.07  19.186724699827245\\
0.08  21.978413610789474\\
0.09  24.51318985345243\\
0.1  26.802503574592695\\
0.11  28.884140258572938\\
0.12  30.77355760354153\\
0.13  32.485640800308005\\
0.14  34.00378713604635\\
0.15  35.33386481097955\\
0.16  36.51480432414793\\
0.17  37.54732130972504\\
0.18  38.48322768187485\\
0.19  39.322094060093235\\
0.2  40.072508054462624\\
0.21  40.738620343189524\\
0.22  41.35320697142186\\
0.23  41.930437495795644\\
0.24  42.477754511715645\\
0.25  42.98642728226472\\
0.26  43.452018875566964\\
0.27  43.86408103268874\\
0.28  44.25052348639794\\
0.29  44.586155913786115\\
0.3  44.89731365243938\\
0.31  45.19802313215903\\
0.32  45.48441992840796\\
0.33  45.716571654302896\\
0.34  45.91651984238873\\
0.35  46.11331924011101\\
0.36  46.2962353348667\\
0.37  46.48072582480417\\
0.38  46.65090363127092\\
0.39  46.82065205723356\\
0.4  46.99798620543567\\
0.41  47.16243893851414\\
0.42  47.310002705097176\\
0.43  47.46529532075439\\
0.44  47.60326958941205\\
0.45  47.73809506770615\\
0.46  47.87363618017378\\
0.47  48.00717351695552\\
0.48  48.150586605332045\\
0.49  48.27567945886606\\
0.5  48.39089656080529\\
0.51  48.502249238207426\\
0.52  48.61546256446075\\
0.53  48.72051766113577\\
0.54  48.818702669744845\\
0.55  48.92146773706455\\
0.56  49.02838348259076\\
0.57  49.13000353523282\\
0.58  49.23176671470957\\
0.59  49.32522853777332\\
0.6  49.42713484408478\\
0.61  49.531760560255684\\
0.62  49.63538438858363\\
0.63  49.73757694856451\\
0.64  49.85708785554495\\
0.65  49.95741976667463\\
0.66  50.05388725326723\\
0.67  50.15164288137218\\
0.68  50.230935147799926\\
0.69  50.300065408963455\\
0.7  50.36332746990401\\
0.71  50.429738321208106\\
0.72  50.50072923122283\\
0.73  50.57172014123756\\
0.74  50.64113665607051\\
0.75  50.718997654151174\\
0.76  50.78412036394292\\
0.77  50.85210561042879\\
0.78  50.916369559212285\\
0.79  50.976769083458684\\
0.8  51.03530795885389\\
0.81  51.08754925352199\\
0.82  51.135926123653\\
0.83  51.19145933551936\\
0.84  51.24742192788984\\
0.85  51.30839395947506\\
0.86  51.36421342501084\\
0.87  51.41230404147243\\
0.88  51.46468846297524\\
0.89  51.512206572097995\\
0.9  51.55671901769191\\
0.91  51.60108833645112\\
0.92  51.637442552466716\\
0.93  51.677804319854125\\
0.94  51.70685906729967\\
0.95  51.747363961521785\\
0.96  51.78815510941332\\
0.97  51.825368086437166\\
0.98  51.85385032654387\\
0.99  51.88490884967531\\
1.0  51.90924041157553\\
1.01  51.93443073448398\\
1.02  51.9530372229959\\
1.03  51.98309385828439\\
1.04  52.00356099564751\\
1.05  52.02460064034946\\
1.06  52.053369134125596\\
1.07  52.08356889624879\\
1.08  52.11720370240496\\
1.09  52.153701045255275\\
1.1  52.178891368163725\\
1.11  52.20994989129517\\
1.12  52.239147765575424\\
1.13  52.26390870797976\\
1.14  52.28280145016109\\
1.15  52.29868852881358\\
1.16  52.31886941250728\\
1.17  52.33303896914329\\
1.18  52.353219852836986\\
1.19  52.37841017574544\\
1.2  52.3937247470591\\
1.21  52.41104309405866\\
1.22  52.42106197248816\\
1.23  52.43222586559531\\
1.24  52.442674124528935\\
1.25  52.45956309102438\\
1.26  52.46872320844563\\
1.27  52.48260651141222\\
1.28  52.49520167286644\\
1.29  52.50765370748597\\
1.3  52.514380668717195\\
1.31  52.523111405634324\\
1.32  52.53685158176621\\
1.33  52.54830172854278\\
1.34  52.560467509492895\\
1.35  52.571345148930625\\
1.36  52.5789308711701\\
1.37  52.585944086070754\\
1.38  52.592671047301984\\
1.39  52.59939800853323\\
1.4  52.6051230819215\\
1.41  52.612422550491566\\
1.42  52.62258455575577\\
1.43  52.63532284404471\\
1.44  52.64634361031716\\
1.45  52.65249806420956\\
1.46  52.65893877177138\\
1.47  52.66165818163081\\
1.48  52.66437759149025\\
1.49  52.6673832550191\\
};


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

